Personalized Popular Music Generation Using Imitation and Structure

Many practices have been presented in music generation recently. While stylistic music generation using deep learning techniques has became the main stream, these models still struggle to generate music with high musicality, different levels of music structure, and controllability. In addition, more application scenarios such as music therapy require imitating more specific musical styles from a few given music examples, rather than capturing the overall genre style of a large data corpus. To address requirements that challenge current deep learning methods, we propose a statistical machine learning model that is able to capture and imitate the structure, melody, chord, and bass style from a given example seed song. An evaluation using 10 pop songs shows that our new representations and methods are able to create high-quality stylistic music that is similar to a given input song. We also discuss potential uses of our approach in music evaluation and music therapy.

==> makefile <==
MAIN= paper
TEXPARTS= 	$(MAIN).tex 		\
		000abstract.tex		\
		010intro.tex 		\
		020survey.tex 		\
		030data.tex		\
		040method.tex 		\
		050experiments.tex 	\
		060conclusions.tex 	\
		099appendix.tex 		

BIBPARTS= BIB/*.bib
FIGPARTS= FIG/*.pdf FIG/*.png
STYPARTS= mdwlist.sty
ALL= makefile  $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) $(STYPARTS) README 

$(MAIN).pdf: $(MAIN).tex
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

clean:
	\rm -f *.dvi *.bbl *.aux *.log *.blg *.toc

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf
	\rm -rf TST
	\rm -f all.tar


all.tar:
	tar cvfh all.tar makefile $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) README 


